Nobel begets Nobel

I construct the professor-student network for laureates of and candidates for the Nobel Prize in Economics. I study the effect of proximity to previous Nobelists on winning the Nobel Prize. Conditional on being Nobel-worthy, students and grandstudents of Nobel laureates are significantly less likely to win. Professors and fellow students of Nobel Prize winners, however, are significantly more likely to win.

==> cand1.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Probability of winning the Nobel Prize.\label{tab:results}}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Probit}\\
\hline
Female              &      -0.242         &       8.228         &      -0.113         &       3.252         \\
      &     (-0.33)         &      (1.82)         &     (-0.40)         &      (1.92)          \\
Distance to Nobel professors      &      1.233\sym{**} &       2.671\sym{*}  &       0.522\sym{**} &       1.253\sym{*}  \\
                    &      (3.03)         &      (2.16)         &      (2.99)         &      (2.20) \\
Distance to Nobel students            &       4.116\sym{***}&       10.94\sym{**} &       2.285\sym{***}&       5.027\sym{**} \\
                    &      (4.53)         &      (2.60)         &      (4.53)         &      (3.17)         \\
\hline
Individual fixed effects & No & Yes & No & Yes \\

Observations        &        4248         &        1827         &        4248         &        1827         \\
\hline\hline
\end{tabular}
\begin{tablenotes}
\textit{t} statistics in parentheses; \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)
\end{tablenotes}
\end{table}

==> candtable.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Probability of winning the Nobel Prize.\label{tab:results}}
\begin{tabular}{l*{8}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}\\
\hline
won                 &                     &                     &                     &                     &                     &                     &                     &                     \\
female              &      -0.985         &      -0.374         &      -0.998         &      -0.395         &      -1.719\sym{*}  &      -0.696\sym{*}  &      -0.871         &      -0.871         \\
                    &     (-1.37)         &     (-1.45)         &     (-1.39)         &     (-1.49)         &     (-2.13)         &     (-2.14)         &     (-1.16)         &     (-1.16)         \\
[1em]
indist              &       0.533         &       0.223         &       0.585         &       0.237         &       0.555         &       0.208         &       0.440         &       0.440         \\
                    &      (1.29)         &      (1.32)         &      (1.41)         &      (1.37)         &      (1.10)         &      (1.00)         &      (0.98)         &      (0.98)         \\
[1em]
outdist             &       3.373\sym{***}&       1.842\sym{***}&       3.769\sym{***}&       1.916\sym{***}&       5.100\sym{***}&       2.380\sym{**} &       3.861\sym{***}&       3.861\sym{***}\\
                    &      (4.26)         &      (4.14)         &      (3.58)         &      (3.83)         &      (3.30)         &      (3.19)         &      (3.34)         &      (3.34)         \\
\hline
Observations        &        4899         &        4899         &        4899         &        4899         &        4245         &        4245         &        4851         &        4851         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}


==> candtabledist.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Probability of winning the Nobel Prize.\label{tab:results}}
\begin{tabular}{l*{8}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{log12}&\multicolumn{1}{c}{prob12}\\
\hline
won                 &                     &                     &                     &                     &                     &                     &                     &                     \\
female              &      -1.060         &      -0.421         &      -0.998         &      -0.395         &      -0.927         &      -0.361         &      -0.238         &      0.0163         \\
                    &     (-1.48)         &     (-1.59)         &     (-1.39)         &     (-1.49)         &     (-1.29)         &     (-1.37)         &     (-0.32)         &      (0.06)         \\
[1em]
indist05            &       0.275         &       0.120         &                     &                     &                     &                     &                     &                     \\
                    &      (0.48)         &      (0.50)         &                     &                     &                     &                     &                     &                     \\
[1em]
outdist05           &       1.864         &       0.981         &                     &                     &                     &                     &                     &                     \\
                    &      (1.12)         &      (1.17)         &                     &                     &                     &                     &                     &                     \\
[1em]
indist              &                     &                     &       0.585         &       0.237         &                     &                     &      -1.907\sym{**} &      -0.799\sym{**} \\
                    &                     &                     &      (1.41)         &      (1.37)         &                     &                     &     (-3.00)         &     (-3.01)         \\
[1em]
outdist             &                     &                     &       3.769\sym{***}&       1.916\sym{***}&                     &                     &       4.259\sym{***}&       2.201\sym{***}\\
                    &                     &                     &      (3.58)         &      (3.83)         &                     &                     &      (3.32)         &      (3.44)         \\
[1em]
indist2             &                     &                     &                     &                     &       0.508         &       0.204         &                     &                     \\
                    &                     &                     &                     &                     &      (1.52)         &      (1.48)         &                     &                     \\
[1em]
outdist2            &                     &                     &                     &                     &       3.943\sym{***}&       1.883\sym{***}&                     &                     \\
                    &                     &                     &                     &                     &      (6.05)         &      (5.67)         &                     &                     \\
[1em]
sibling             &                     &                     &                     &                     &                     &                     &       11.59\sym{***}&       5.522\sym{***}\\
                    &                     &                     &                     &                     &                     &                     &     (13.46)         &     (13.65)         \\
\hline
Observations        &        4899         &        4899         &        4899         &        4899         &        4899         &        4899         &        4899         &        4899         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}


==> candtablelimit.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Probability of winning the Nobel Prize.\label{tab:results}}
\begin{tabular}{l*{8}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}\\
\hline
won                 &                     &                     &                     &                     &                     &                     &                     &                     \\
female              &      -0.998         &      -0.395         &      -0.749         &      -0.303         &      -0.778         &      -0.317         &       8.228         &       3.252         \\
                    &     (-1.39)         &     (-1.49)         &     (-1.04)         &     (-1.10)         &     (-1.08)         &     (-1.15)         &      (1.82)         &      (1.92)         \\
[1em]
indist              &       0.585         &       0.237         &       0.511         &       0.211         &       0.595         &       0.245         &       2.671\sym{*}  &       1.253\sym{*}  \\
                    &      (1.41)         &      (1.37)         &      (1.24)         &      (1.21)         &      (1.45)         &      (1.41)         &      (2.16)         &      (2.20)         \\
[1em]
outdist             &       3.769\sym{***}&       1.916\sym{***}&       3.564\sym{***}&       1.834\sym{***}&       3.565\sym{***}&       1.827\sym{***}&       10.94\sym{**} &       5.027\sym{**} \\
                    &      (3.58)         &      (3.83)         &      (3.40)         &      (3.64)         &      (3.40)         &      (3.63)         &      (2.60)         &      (3.17)         \\
\hline
Observations        &        4899         &        4899         &        4432         &        4432         &        4340         &        4340         &        1912         &        1912         \\
\hline\hline
\multicolumn{9}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{9}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}


==> candtablesplit.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Probability of winning the Nobel Prize.\label{tab:split}}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}&\multicolumn{1}{c}{Logit}&\multicolumn{1}{c}{Probit}\\
\hline
won                 &                     &                     &                     &                     &                     &                     \\
female              &      -0.998         &      -0.395         &      -1.002         &      -0.393         &      -1.002         &      -0.393         \\
                    &     (-1.39)         &     (-1.49)         &     (-1.39)         &     (-1.48)         &     (-1.39)         &     (-1.48)         \\
[1em]
indist              &       0.585         &       0.237         &                     &                     &                     &                     \\
                    &      (1.41)         &      (1.37)         &                     &                     &                     &                     \\
[1em]
outdist             &       3.769\sym{***}&       1.916\sym{***}&       3.666\sym{***}&       1.874\sym{***}&       3.666\sym{***}&       1.874\sym{***}\\
                    &      (3.58)         &      (3.83)         &      (3.49)         &      (3.73)         &      (3.49)         &      (3.73)         \\
[1em]
indistlive          &                     &                     &       0.254         &       0.102         &                     &                     \\
                    &                     &                     &      (0.61)         &      (0.60)         &                     &                     \\
[1em]
indistdead          &                     &                     &       0.837         &       0.362         &                     &                     \\
                    &                     &                     &      (1.80)         &      (1.79)         &                     &                     \\
[1em]
indistremote        &                     &                     &                     &                     &       0.837         &       0.362         \\
                    &                     &                     &                     &                     &      (1.80)         &      (1.79)         \\
[1em]
indistrecent        &                     &                     &                     &                     &       0.254         &       0.102         \\
                    &                     &                     &                     &                     &      (0.61)         &      (0.60)         \\
\hline
Observations        &        4899         &        4899         &        4899         &        4899         &        4899         &        4899         \\
\hline\hline
\multicolumn{7}{l}{\footnotesize \textit{t} statistics in parentheses}\\
\multicolumn{7}{l}{\footnotesize \sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
\end{table}

